A rational approximation method for solving acoustic nonlinear eigenvalue problems

We present two approximation methods for computing eigenfrequencies and eigenmodes of large-scale nonlinear eigenvalue problems resulting from boundary element method (BEM) solutions of some types of acoustic eigenvalue problems in three-dimensional space. The main idea of the first method is to approximate the resulting boundary element matrix within a contour in the complex plane by a high accuracy rational approximation using the Cauchy integral formula. The second method is based on the Chebyshev interpolation within real intervals. A Rayleigh-Ritz procedure, which is suitable for parallelization is developed for both the Cauchy and the Chebyshev approximation methods when dealing with large-scale practical applications. The performance of the proposed methods is illustrated with a variety of benchmark examples and large-scale industrial applications with degrees of freedom varying from several hundred up to around two million.

==> analysis.tex <==
\section{Theoretical investigation}
%%%%
The following result gives a bound for the error obtained when using 
the trapezoidal rule to approximate the interal \eqref{eq:Tz}.
\begin{theorem}\cite[Thm. 13.2]{TefW14}
%
Suppose $T$ is analytic and bounded in the disk $|z| < r$ for some $r > 1$,
and $\widetilde T(\lambda)$ is the approximation to $T(\lambda)$ for some $|\lambda|<1$ obtained by applying the $m$-point trapezoidal rule on the unit circle to
\[
T(\lambda) = \frac{1}{2\pi\imath} \int_{|z|=1} \frac{T(z)}{z - \lambda} dz.
\]
%%YS I assume this is $m \rightarrow \infty$, not $m \rightarrow 0$,
Then as $m \rightarrow \infty$,
\[
T(\lambda) - \widetilde T(\lambda) = \mathcal{O}(\max\{r^{-m},|\lambda|^m\}).
\]
\end{theorem}

The integral form for the representation of the difference between an analytic function $f$ and its approximation $p$ is given as
%
\[
f(t) - p(t) = \frac{A(t)}{2\pi\imath} \int_{\Gamma} \frac{f(z)}{A(z)(z-t)} \ dz.
\]
The form of the approximation $p$ depends on the zeros of the so-called 
``auxiliary" function $A(z)$, which are interior to the curve. If we choose
\[
A(z) = \frac{\prod_{i=0}^{n}(z - \beta_i)}{\prod_{i=1}^{n}(z-\alpha_i)},
\]
then $p$ is the rational approximation function which agrees with $f(t)$
at each point  $t = \beta_i$  and has poles at each point $t = \alpha_i$ [Walsh's Rational
Approximation, 15, p. 186].

==> qr.tex <==
\newpage

\section*{Solving Linear Systems with QR Factorization}

Supposed we are interested in solving a linear sysem
%
\[
Ax = b,
\]
%
with nonsingular matrix $A \in \F^{n \times n}$ and vector $b \in \F^n$.
To do so, we replace $A$ with its QR factorization,
%
\[
QRx = b.
\]
Since the columns of $Q$ are orthonormal $Q^*Q = I$ yields
%
\[
Q^*QRx = Rx =  Q^*b.
\]
%
Since $R$ is an upper triangular matrix, system $Rx = Q^*b$ can be solved using
back-substitution. We can formally write the solution of \eqref{} as
%
\[
x = R^{-1}Q^*b.
\]
%
Note: Since the columns of $A$ are linearly independent, the diagonal entries of $R$ obtained via the Gram-Schmidt
process are always nonzero, so $R$ is nonsingular.






